Atomic Hydrogen Properties of AGN Host Galaxies: HI in 16 NUclei of GAlaxies (NUGA) Sources

We present a comprehensive spectroscopic imaging survey of the distribution and kinematics of atomic hydrogen (HI) in 16 nearby spiral galaxies hosting low luminosity AGN, observed with high spectral and spatial resolution (resolution: ~20 arcsec, 5 km/s) using the NRAO Very Large Array (VLA). The sample contains a range of nuclear types, ranging from Seyfert to star-forming nuclei and was originally selected for the NUclei of GAlaxies project (NUGA) - a spectrally and spatially resolved interferometric survey of gas dynamics in nearby galaxies designed to identify the fueling mechanisms of AGN and the relation to host galaxy evolution. Here we investigate the relationship between the HI properties of these galaxies, their environment, their stellar distribution and their AGN type. The large-scale HI morphology of each galaxy is classified as ringed, spiral, or centrally concentrated; comparison of the resulting morphological classification with AGN type reveals that ring structures are significantly more common in LINER than in Seyfert host galaxies, suggesting a time evolution of the AGN activity together with the redistribution of the neutral gas. Dynamically disturbed HI disks are also more prevalent in LINER host galaxies than in Seyfert host galaxies. While several galaxies are surrounded by companions (some with associated HI emission), there is no correlation between the presence of companions and the AGN type (Seyfert/LINER).

==> bib.tex <==
@INPROCEEDINGS{1992ASPC...25..131V,
   author = {{van der Hulst}, J.~M. and {Terlouw}, J.~P. and {Begeman}, K.~G. and 
	{Zwitser}, W. and {Roelfsema}, P.~R.},
    title = "{The Groningen Image Processing SYstem, GIPSY}",
booktitle = {ASP Conf. Ser.  25: Astronomical Data Analysis Software and Systems I},
     year = 1992,
   editor = {{Worrall}, D.~M. and {Biemesderfer}, C. and {Barnes}, J.},
    pages = {131-+},
   adsurl = {http://adsabs.harvard.edu/cgi-bin/nph-bib_query?bibcode=1992ASPC...25..131V&db_key=AST},
  adsnote = {Provided by the Smithsonian/NASA Astrophysics Data System}
}
